Learning Representational Invariances for Data-Efficient Action Recognition

Data augmentation is a ubiquitous technique for improving image classification when labeled data is scarce. Constraining the model predictions to be invariant to diverse data augmentations effectively injects the desired representational invariances to the model (e.g., invariance to photometric variations) and helps improve accuracy. Compared to image data, the appearance variations in videos are far more complex due to the additional temporal dimension. Yet, data augmentation methods for videos remain under-explored. This paper investigates various data augmentation strategies that capture different video invariances, including photometric, geometric, temporal, and actor/scene augmentations. When integrated with existing semi-supervised learning frameworks, we show that our data augmentation strategy leads to promising performance on the Kinetics-100/400, Mini-Something-v2, UCF-101, and HMDB-51 datasets in the low-label regime. We also validate our data augmentation strategy in the fully supervised setting and demonstrate improved performance.

==> cviu_highlight.tex <==
\thispagestyle{empty}

\ifpreprint
  \vspace*{-1pc}
\else
\fi

\begin{table*}[!t]
\ifpreprint\else\vspace*{-15pc}\fi

\section*{Research Highlights (Required)}

\vskip1pc

\fboxsep=6pt
\fbox{
\begin{minipage}{.95\textwidth}
\vskip1pc
\begin{itemize}

\item We study various types of strong video data augmentation strategies for data-efficient action recognition.
\item We introduce a novel scene augmentation strategy, ActorCutMix, to encourage the scene invariance, which is crucial for the action recognition.
\item Our strong data augmentation strategies significantly improve the data efficiency in both the semi-supervised and fully-supervised learning settings, achieving promising results in standard video action recognition benchmarks. 
\item Our source code and pre-trained models are publicly available at \url{https://github.com/vt-vl-lab/video-data-aug}.

\end{itemize}
\vskip1pc
\end{minipage}
}

\end{table*}

==> cviu_optional.tex <==
\thispagestyle{empty}
\ifpreprint
  \vspace*{-1pc}
\fi

\begin{table*}[!th]
\ifpreprint\else\vspace*{-5pc}\fi

\section*{Graphical Abstract (Optional)}
To create your abstract, please type over the instructions in the
template box below.  Fonts or abstract dimensions should not be changed
or altered. 

\vskip1pc
\fbox{
\begin{tabular}{p{.4\textwidth}p{.5\textwidth}}
\bf Learning Representational Invariances for Data-Efficient Action Recognition  \\
Yuliang Zou, Jinwoo Choi, Qitong Wang, Jia-Bin Huang \\[1pc]
& 
Data augmentation is a ubiquitous technique for improving image classification when labeled data is scarce.
Constraining the model predictions to be invariant to diverse data augmentations effectively injects the desired representational invariances to the model (e.g., invariance to photometric variations) and helps improve accuracy.
Compared to image data, the appearance variations in videos are far more complex due to the additional temporal dimension.
Yet, data augmentation methods for videos remain under-explored.
This paper investigates various data augmentation strategies that capture different video invariances, including photometric, geometric, temporal, and actor/scene augmentations.
When integrated with existing semi-supervised learning frameworks, we show that our data augmentation strategy leads to promising performance on the Kinetics-100/400, Mini-Something-v2, UCF-101, and HMDB-51 datasets in the low-label regime.
We also validate our data augmentation strategy in the fully supervised setting and demonstrate improved performance.
\end{tabular}
}

\end{table*}

==> figure/fig_confmat_actorcutmix.tex <==
\begin{figure*}[ht]
    \centering
    \mpage{0.950}{\includegraphics[width=\linewidth]{figure/img_files/confmat_actorcutmix_only_sorted.jpg}}
    \mpage{0.950}{    (c) ActorCutMix augmentation only }
    \vspace{-3mm}
    \label{fig:conf_acm}
\end{figure*}


==> figure/fig_confmat_all.tex <==
\begin{figure*}
    \centering
    \mpage{0.950}{\includegraphics[width=\linewidth]{figure/img_files/confmat_final_sorted.jpg}}
    \mpage{0.950}{    (d) All augmentations }
    \figcaption{UCF-101 $20\%$ label split confusion matrix visualization}{We compare the confusion matrices of the i) supervised baseline, and our semi-supervised models with ii) temporal augmentation only, iii) ActorCutMix only, and iv) all augmentations. We sort the classes in ascending order of the baseline accuracy. Best viewed with zoom and color.}
    \label{fig:conf_all}
\end{figure*}


==> figure/fig_confmat_baseline.tex <==
\begin{figure*}
    \centering
    \mpage{0.950}{\includegraphics[width=\linewidth]{figure/img_files/confmat_baseline_sorted.jpg}}
    \mpage{0.950}{    (a) Supervised baseline    }
    \vspace{-3mm}
    \label{fig:conf_baseline}
\end{figure*}


==> figure/fig_confmat_temp.tex <==
\begin{figure*}
    \centering
    \mpage{0.950}{\includegraphics[width=\linewidth]{figure/img_files/confmat_tempaug_only_sorted.jpg}}
    \mpage{0.950}{    (b) Temporal augmentations only }
    \vspace{-3mm}
    \label{fig:conf_temp}
\end{figure*}


==> overview.tex <==
\section{Overview}
\label{sec:overview}


\input{figure/fig_overview}

==> sup_content.tex <==
In this supplementary material, we present more implementation details and experimental results to complement the main paper.

\section{Implementation Details}
We use SGD with momentum as our optimizer, with an initial learning rate of $0.2$, a momentum value of $0.9$, and a weight decay value of $1e-4$.
We use the cosine annealing policy for learning rate decay.
We also adopt the synchronous batch normalization across eight GPUs.
For the UCF-101 dataset~\cite{soomro2012ucf101} and Kinetics-100 dataset~\cite{jing2020videossl,kay2017kinetics}, we train our method for 360 epochs with respect to unlabeled data.
For the HMDB-51 dataset~\cite{kuehne2011hmdb}, we train our method for 600 epochs with respect to unlabeled data.
We list the values of the other hyper-parameters as below.
\input{table/hyper}


\section{Algorithm Outline}
We provide the algorithm outline of our strong data augmentation strategy for video in \algref{alg:aug}.
\input{table/algorithm}

\section{More Ablation Experiments}
We show more ablation results on the $20\%$ label split of the UCF-101 using a R(2+1)D ResNet-34 model.

\topic{Strong augmentation on the labeled branch.}
Currently, the \emph{strong} data augmentation is only applied to the unlabeled branch by default, as shown in Figure~\red{1} of the main paper.
Here, we conduct an experiment applying the strong augmentation on the labeled branch as well.
It achieves a similar performance (56.46\%) as our default setting (56.73\%).
We conjecture that the strong augmentations have already injected the visual invariances in the unlabeled branch. 
Additional strong augmentation for the labeled branch may not add more visual invariances to the model.
Therefore, the performance difference is negligible.
For better training efficiency, we choose to use the default setting.

\topic{Different initialization.}
We investigate whether our strong data augmentation strategy
can still improve over the supervised baseline, given strong pre-trained model weights as an initialization. %
As shown in \tabref{abl_init}, while the improvement over the supervised baseline is not as significant as the boost in the train-from-scratch setting, the proposed method can still achieve a sizable improvement (72.40\% $\rightarrow$ 77.37\%).
The results validate the general applicability of the strong data augmentation in practical scenarios.
\input{table/abl_init}


\section{ImageNet Knowledge Distillation}
As discussed in Section~\red{4.3} of the main paper, we hypothesize that the ImageNet knowledge distillation in VideoSSL~\cite{jing2020videossl} may be the key factor to its good performance in the extremely low label ratios (10\% and 5\%) on the UCF-101 dataset.
In this section, we aim to explore whether an additional knowledge distillation loss can complement our strong data augmentations and whether it would lead to improved performance.
Following VideoSSL~\cite{jing2020videossl}, we adopt an ImageNet pre-trained ResNet-18 to compute a $1,000$ dimensional ImageNet class probability vector for each frame of all the training videos offline.
Accordingly, we add an additional classification head to predict the ImageNet probability of each video clip on top of the feature extraction backbone.
We randomly select one frame from each (weakly-augmented) video clip during training time and then use its corresponding ImageNet probability as a soft pseudo label for a cross-entropy loss.
The soft pseudo label provides an additional supervisory signal to the feature backbone.
\input{table/kd_all}

As shown in \tabref{kd_all}, our method's performance significantly improves with ImageNet distillation compared to our method without ImageNet distillation ($26.1\%\rightarrow49.5\%$ in $5\%$ label split and $39.9\%\rightarrow52.7\%$ in $10\%$ label split of the UCF-101 dataset).
Our method with ImageNet distillation shows a favorable performance when compared to VideoSSL~\cite{jing2020videossl}.



\section{Additional Results in Low-Label Settings}
This section shows full results to complement Table~\red{2} of the main paper by adding results from other backbones and comparisons with self-supervised learning methods.
With the same amount of data, one can pre-train the model using all the available data (using self-supervised learning) and then fine-tune the model with the small amount of labeled data, instead of conducting semi-supervised learning.
Thus, we establish another type of baselines by fine-tuning the self-supervised video pre-trained models on the labeled data.
We choose two recent state-of-the-art self-supervised methods for video representation, \ie, VCOP~\cite{xu2019self} and DPC~\cite{han2019video}.
As shown in \tabref{main_kinetics}, \tabref{main_ucf}, and \tabref{main_hmdb}, our method achieves promising results when comparing with these self-supervised approaches across three datasets.
\input{table/main_kinetics}

\input{table/main_ucf}

\input{table/main_hmdb}


\section{Improvement over Supervised Baseline and Error Analysis}
In this section, we plug our strong data augmentation into FixMatch~\cite{sohn2020fixmatch} and compare it with the supervised baseline, where only labeled video data is used during training (labeled branch only in Figure~\red{2} of the main paper). Note that we train both our model and the supervised baseline from scratch. As shown in \figref{improve_baseline}, our method consistently outperforms the supervised baseline by a large margin across different label ratios in both the UCF-101 and HMDB-51 datasets.
The performance improvement highlights the efficacy of injecting video representational invariances with our strong data augmentation strategy.

\input{figure/fig_improve_baseline}

\input{figure/fig_class_accuracy}
In \figref{cls_acc}, we visualize the class accuracy curves of the supervised baseline (\red{red} curve) and our semi-supervised model (\blue{blue} curves) with our (i) temporal augmentations only, 
(ii) ActorCutMix augmentation only, and 
(iii) final all augmentations, on 20\% label split of the UCF-101 dataset. 
We sort the classes in ascending order of the baseline accuracy.
We also visualize UCF-101 ($20\%$ label ratio) confusion matrices of the 
(i) supervised baseline, and our semi-supervised models with 
(ii) temporal augmentation only, (iii) ActorCutMix only, and 
(iv) all augmentations (\ie photometric, geometric, temporal, and scene) in \figref{conf_all}. 


Temporal augmentations can reduce the error rate for the classes such as ``BodyWeightSquats" and ``Haircut". 
The baseline model confused ``BodyWeightSquats" with ``TableTennisShot". 
However, our temporal augmentation reduces this type of error significantly ($26.7\% \rightarrow 13.3\%$). 
Temporal augmentations such as T-Half and T-Drop are essentially providing a model less information. 
Therefore, they could encourage the model to focus more on the fine-grained details related to human actions, such as human pose. 
Compared to the baseline, ActorCutMix reduces the error rates of classes such as ``BlowDryHair" and ``ShotPut". 
The baseline is confused the classes ``BlowDryHair" with ``ApplyLipstick," which has similar scenes, \eg, bedroom and restroom. 
In contrast, ActorCutMix significantly reduces this type of error, ($18.4\% \rightarrow 7.9\%$). 
The results imply that ActorCutMix provides various scenes and results in scene invariance of our model. 
Additional invariances to photometric/geometric transformations help our model not to use shortcuts.
Using all augmentations significantly reduces the error rate of the baseline for the class ``PlayingDaf" with ``PlayingFlute" ($26.8\% \rightarrow 4.9\%$).


\clearpage
\input{figure/fig_confmat_baseline}
\input{figure/fig_confmat_temp}
\input{figure/fig_confmat_actorcutmix}
\input{figure/fig_confmat_all}



\section{Improving Fully-Supervised Learning with Cross-Dataset Semi-Supervised Learning}
Lastly, we show that our strong data augmentation strategy can be used in a cross-dataset semi-supervised learning setting to further improve the fully-supervised models.
We use the full training set of the UCF-101 or HMDB-51 datasets as the labeled set, and the Kinetics-100 dataset as the unlabeled set.
Since there is no overlap between the labeled and unlabeled data, we modify the semi-supervised framework (as shown in Figure~\red{2} of the main paper) by replacing the standard/weak augmentation in the labeled branch with our strong data augmentation to make sure we generate diverse samples for both labeled and unlabeled data.

\input{table/ssl_cross}
As shown in \tabref{ssl_cross}, our strong augmentation can be used in a cross-dataset setting (high-data regime), leading to a substantial performance gain comparing to the fully supervised training setting with standard/weak data augmentations.




==> table/kd_all.tex <==
\begin{table*}[ht]
\centering

\caption{\tb{Effect of ImageNet knowledge distillation.}
All the methods use a 3D ResNet-18 model.
The best performance is in \best{bold} and the second best is \second{underlined}.
}


\begin{tabular}{lcccccccccccc}
\toprule
& w/ ImageNet & \multicolumn{2}{c}{Kinetics-100} && \multicolumn{4}{c}{UCF-101} && \multicolumn{3}{c}{HMDB-51}\\
\cmidrule{3-4}
\cmidrule{6-9}
\cmidrule{11-13}
Method & distillation && 20\% && 50\% & 20\% & 10\% & 5\% && 60\% & 50\% & 40\% \\
\midrule
VideoSSL~\citep{jing2020videossl} & \checkmark 
&& 57.7 && 54.3 & 48.7 & \second{42.0} & \second{32.4}
&& 37.0 & 36.2 & 32.7
\\
Ours & - 
&& \second{61.2} && \second{59.9} & \second{51.7} & 40.2 & 27.0
&& \second{38.9} & \second{38.2} & \second{32.9}
\\
Ours & \checkmark 
&& \best{68.7} && \best{64.7} & \best{57.4} & \best{53.0} & \best{45.1}
&& \best{40.8} & \best{39.5} & \best{35.7}    %
\\
\bottomrule
\end{tabular}



\label{tab:kd_all}
\end{table*}


==> table/main_hmdb.tex <==
\begin{table*}[htbp]
\centering

\caption{\tb{Results on HMDB-51.}
The best performance is in \best{bold} and the second best is \second{underlined}.
}

\begin{tabular}{lcccc}
\toprule
&& \multicolumn{3}{c}{Label ratio (\%)} \\
\cmidrule{3-5}
Method & Network & 60 & 50 & 40  \\
\midrule
PL~\citep{lee2013pseudo} & 3D ResNet-18 & 33.5 & 32.4 & 27.3 \\
MT~\citep{tarvainen2017mean} & 3D ResNet-18 & 32.2 & 30.4 & 27.2 \\
S4L~\citep{zhai2019s4l} & 3D ResNet-18 & 35.6 & 31.0 & 29.8 \\
VideoSSL~\cite{jing2020videossl} & 3D ResNet-18 & 37.0 & 36.2 & 32.7 \\
\midrule
VCOP~\citep{xu2019self} & R(2+1)D ResNet-10 & 27.8 & 26.5 & 25.7 \\
DPC~\citep{han2019video} & R(2+3)D ResNet-18 & 37.2 & 33.2 & 31.6 \\
MemDPC~\citep{han2020memory} & R(2+3)D ResNet-18 & 40.6 & 32.8 & 29.7 \\
\midrule
Ours & 3D ResNet-18 & 38.9 & 38.2 & 32.9 \\
Ours & R(2+1)D ResNet-18 & \best{42.5}  & \best{39.5} & \second{33.0} \\
Ours & R(2+1)D ResNet-34 & \second{41.7} & \second{39.2} & \best{34.6} \\
\bottomrule
\end{tabular}






\label{tab:main_hmdb}
\end{table*}


==> table/main_kinetics.tex <==
\begin{table*}[htbp]
\centering

\caption{\tb{Results on Kinetics-100.}
Due to computing resource constraint, we only compare under the 20\% label ratio.
The best performance is in \best{bold} and the second best is \second{underlined}.
}
\vspace{-3mm}


\begin{tabular}{lcc}
\toprule
&& Label ratio (\%) \\
Method & Network & 20   \\
\midrule
PL~\citep{lee2013pseudo} &  3D ResNet-18 & 48.0 \\
MT~\citep{tarvainen2017mean} & 3D ResNet-18 & 47.1 \\
S4L~\citep{zhai2019s4l} & 3D ResNet-18 & 51.1 \\
VideoSSL~\citep{jing2020videossl} & 3D ResNet-18 & 57.7 \\
\midrule
VCOP~\citep{xu2019self} & R(2+1)D ResNet-10 & 50.9 \\
DPC~\citep{han2019video} & R(2+3)D ResNet-34 & 59.2 \\
MemDPC~\citep{han2020memory} & R(2+3)D ResNet-18 & 48.5 \\
\midrule
Ours & 3D ResNet-18 & \second{61.2} \\
Ours & R(2+1)D ResNet-34 & \best{65.8} \\
\bottomrule
\end{tabular}





\label{tab:main_kinetics}
\end{table*}


==> table/main_ucf.tex <==
\begin{table*}[htbp]
\centering

\caption{\tb{Results on UCF-101.}
The best performance is in \best{bold} and the second best is \second{underlined}.
}


\begin{tabular}{lccccc}
\toprule
&& \multicolumn{4}{c}{Label ratio (\%)} \\
\cmidrule{3-6}
Method & Network & 50 & 20 & 10 & 5  \\
\midrule
PL~\citep{lee2013pseudo} & 3D ResNet-18 & 47.5 & 37.0 & 24.7 & 17.6 \\
MT~\citep{tarvainen2017mean} & 3D ResNet-18 & 45.8 & 36.3 & 25.6 & 17.5 \\
S4L~\citep{zhai2019s4l} & 3D ResNet-18 & 47.9 & 37.7 & 29.1 & 22.7 \\
VideoSSL~\citep{jing2020videossl} & 3D ResNet-18 & 54.3 & 48.7 & \best{42.0} & \best{32.4} \\
\midrule
VCOP~\citep{xu2019self} & R(2+1)D ResNet-10 & \second{67.9} & \second{53.1} & 31.1 & 14.4 \\
DPC~\citep{han2019video} & R(2+3)D ResNet-18 & 53.1 & 38.9 & 25.3 & 19.2 \\
MemDPC~\citep{han2020memory} & R(2+3)D ResNet-18 & 60.5 & 47.8 & 31.2 & 27.3 \\
\midrule
Ours & 3D ResNet-18 & 59.9 & 51.7 & \second{40.2} & \second{27.0} \\
Ours & R(2+1)D ResNet-18 & 64.2 & 52.5 & 39.9  & 26.1 \\
Ours & R(2+1)D ResNet-34 & \best{68.7} & \best{56.7} & 39.7 & 22.8 \\
\bottomrule
\end{tabular}





\label{tab:main_ucf}
\end{table*}

